Kwai Summary Attention Technical Report

Long-context ability, has become one of the most important iteration direction of next-generation Large Language Models, particularly in semantic understanding/reasoning, code agentic intelligence and recommendation system. However, the standard softmax attention exhibits quadratic time complexity with respect to sequence length. As the sequence length increases, this incurs substantial overhead in long-context settings, leading the training and inference costs of extremely long sequences deteriorate rapidly. Existing solutions mitigate this issue through two technique routings: i) Reducing the KV cache per layer, such as from the head-level compression GQA, and the embedding dimension-level compression MLA, but the KV cache remains linearly dependent on the sequence length at a 1:1 ratio. ii) Interleaving with KV Cache friendly architecture, such as local attention SWA, linear kernel GDN, but often involve trade-offs among KV Cache and long-context modeling effectiveness. Besides the two technique routings, we argue that there exists an intermediate path not well explored: {Maintaining a linear relationship between the KV cache and sequence length, but performing semantic-level compression through a specific ratio $k$}. This $O(n/k)$ path does not pursue a ``minimum KV cache'', but rather trades acceptable memory costs for complete, referential, and interpretable retention of long distant dependency. Motivated by this, we propose Kwai Summary Attention (KSA), a novel attention mechanism that reduces sequence modeling cost by compressing historical contexts into learnable summary tokens.

==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}




==> sections/exp_part_renl.tex <==
\subsubsection{Model Hyper-parameters Configuration}

We evaluate different attention architectures under two experimental settings: train-from-scratch and continual-pretraining (CPT).

% \paragraph{Train-from-Scratch experiments.} 
% We train a 1.6B parameter language model with structure in Table~\ref{tab:Model_Configuration} and adopt the following architectures as baselines: 
% \textbf{pure full attention}, \textbf{pure summary attention}, and four hybrid variants: 
% \textbf{GDN+Full}, \textbf{Summary+Full}, \textbf{Sliding Chunk+Full}, and \textbf{Sliding Window+Full}, all with a \textbf{3:1 mixing ratio}.
% Training follows a progressive sequence length extension strategy: models are first trained on 250B tokens at a sequence length of 8K,
% followed by continued training on 50B tokens each at 32K, 64K, and 128K,
% amounting to 400B tokens in total.

% \paragraph{Continue-Pretraining experiments.}
% We conduct training from a 4B checkpoint as in Table~\ref{tab:Model_Configuration} and compare with: \textbf{Full Attention}, \textbf{Full Summary}, \textbf{Summary+Full}, \textbf{Sliding Chunk+Full}, \textbf{Sliding Window+Full}, and \textbf{Linear+Full} with \textbf{mixing ratio 3:1}. 
% Specifically, for CPT experiments, we feature a \textbf{hybrid ring-linear attention}~\cite{team2025every} architecture, interleaving simple Gated Linear Attention (GLA)~\cite{yang2024fla} with  full attention layers in a 3:1 ratio.
% Specifically, every fourth layer is designated as a full attention layer, while the remaining three are implemented via the \texttt{chunk\_simple\_gla} kernel.
% The long-context extension schedule consists of 25B, 35B, and 15B tokens at sequence lengths of 32K, 64K, and 128K respectively, adding up to 75B tokens. 


\paragraph{Train-from-Scratch experiments.}
We train a 1.6B parameter language model with the architecture detailed in Table~\ref{tab:Model_Configuration} and compare the following configurations:
\textbf{pure full attention}, \textbf{pure summary attention}, and four hybrid variants---
\textbf{GDN+Full}, \textbf{Summary+Full}, \textbf{Sliding Chunk+Full}, and \textbf{Sliding Window+Full}---all with a \textbf{3:1 mixing ratio}.
Training follows a progressive length-extension schedule: models are first trained on 250B tokens at a sequence length of 8K, then further trained on 50B tokens each at 32K, 64K, and 128K, resulting in a total of 400B tokens.

\paragraph{Continual-Pretraining experiments.}
We initialize from a 4B checkpoint (Table~\ref{tab:Model_Configuration}) and compare against:
\textbf{Full Attention}, \textbf{Full Summary}, \textbf{Summary+Full}, \textbf{Sliding Chunk+Full}, \textbf{Sliding Window+Full}, and \textbf{Linear+Full}, all at a \textbf{3:1 mixing ratio}.
For the CPT setup, we adopt a \textbf{hybrid ring-linear attention} architecture~\cite{team2025every} that interleaves simple Gated Linear Attention (GLA)~\cite{yang2024fla} with full attention layers.
Specifically, every fourth layer is a full attention layer and the remaining three use the \texttt{chunk\_simple\_gla} kernel.
We use 25B, 35B, and 15B tokens at sequence lengths of 32K, 64K, and 128K for training, respectively, totaling 75B tokens.


\begin{figure*}[t]
\centering
\includegraphics[width=0.99\textwidth]{figures/dataset.pdf}
% 中文：预训练数据配比的整体分布。
\caption{Overall Distribution of Pretraining Data Proportions.}
\label{fig:datasets_distribution}
\end{figure*}

\subsubsection{Datasets Pipeline}
% 中文：预训练语料由六个关键数据类别组成：Common Knowledge、Math、Code、STEM、
% General Reasoning 和 Long Context。该数据配比的详细构成如图~\ref{fig:datasets_distribution} 所示。
The pretraining corpus is composed of six categories: Common Knowledge, Math, Code, STEM, General Reasoning, and Long Context. 
A comprehensive breakdown of data formulation is in Figure~\ref{fig:datasets_distribution}.


\textbf{Long Context} is a primary data class, as it directly serves our goal of reinforcing the model's long-sequence modeling capacity.
We construct a hybrid mixture tailored for context-length extension by combining naturally long documents, \textit{i.e.,} books, long-form QA across code, math, and STEM; 
with synthetic sequences that probe long-range information tracking.
We further incorporate structured benchmark-style sequences from long-context evaluation tasks to ensure robustness.

\textbf{Common Knowledge} forms the foundational layer, sourced from diverse high-quality web text~\cite{penedo2024fineweb}, educational content, and curated open-source corpora. 
The sources span filtered CommonCrawl snapshots~\cite{su2025nemotron}, web-extracted educational material, and high-quality open-domain text, ensuring broad coverage of general world knowledge.

\textbf{Math} and \textbf{Code} are constructed from both natural and synthetic sources.
The math subset integrates web-crawled mathematical content, competition problems, Chinese-language resources, and QA pairs, augmented with synthetic problem, \textit{i.e.,} solution sequences to improve coverage of rare reasoning patterns.
The code subset combines GitHub repositories, competition solutions, code-related QA pairs, and synthetic generation tasks spanning multiple programming languages.

\textbf{STEM} and \textbf{General Reasoning} broaden the model's domain expertise through academic papers, textbook-style content, encyclopedia entries, long-form books, and structured QA corpora.
Domain-specific scientific documents and exam-style data further strengthen coverage of technical disciplines.


% 中文：训练流程采用统一的固定数据配比（如图~\ref{fig:datasets_distribution} 所示），
% 并在该配比之上按阶段逐步扩展上下文长度。训练首先在 8K 上下文窗口下进行，随后依次在
% 32K、64K 和 128K 长度下继续训练，每个阶段消费该固定配比中对应的一部分数据后再进入下一阶段。
% 这种设置让模型先在短上下文阶段建立稳健的基础能力，再在不改变底层数据配比的前提下渐进地
% 适应更长的序列。图中占主导的 Long Context 子集，提供了支撑这一渐进式长度扩展所需的
% 自然长文档以及合成长序列；其余类别则在所有阶段中持续为模型补充知识、推理、代码、数学
% 和 STEM 等方面的广度覆盖。
The training pipeline follows the data mixture ratios shown in Figure~\ref{fig:datasets_distribution} and progressively extends the context length across stages.
In train-from-scratch experiments, the context length increases from 8K to 32K, 64K, and finally 128K tokens.
In CPT experiments, training starts directly at 32K and advances to 128K, with all stages using the same ratios of data classes mixture.

\subsubsection{Evaluation Benchmark}
We categorize the evaluation benchmarks into two groups, targeting long-context modeling 
ability and general language capability accordingly.

\textbf{Long-Context Benchmarks:} 
RULER~\cite{hsiehruler} is a comprehensive long-context evaluation suite that 
assesses models across multiple dimensions including retrieval, multi-hop tracing, 
aggregation, and question answering, with configurable context lengths up to 128K tokens. 
LongBench v2~\cite{bai2025longbench} provides a challenging set of long-document 
understanding tasks covering diverse domains and realistic long-context scenarios, serving 
as a robust testbed for evaluating the practical long-context capabilities of language models.

\textbf{General Capability Benchmarks:} 
MMLU~\cite{hendrycksmeasuring} is a widely adopted benchmark spanning 57 subjects across 
STEM, humanities, and social sciences, evaluating the breadth of world knowledge and 
reasoning ability. CMMLU~\cite{li2024cmmlu} is its Chinese-language counterpart, 
assessing knowledge understanding across diverse domains in Chinese. 
GSM8K~\cite{cobbe2021training} evaluates grade-school mathematical reasoning through 
multi-step arithmetic problem solving. CMATH~\cite{wei2023cmath} further assesses 
mathematical reasoning ability in Chinese, covering elementary to competition-level 
problems. MBPP~\cite{austin2021program} benchmarks code generation capability by requiring 
models to synthesize short Python programs from natural language descriptions.

\subsubsection{Training Recipes}

To adapt  summary attention with existing model architecture seamlessly, we devise a three stage training curriculum that features warm-up, parameter annealing, and sequence length extension:

\paragraph{Warm-up of KSA.} 




\paragraph{Parameter annealing.} 




\paragraph{Sequence length extension.} 







==> sections/introduction.tex <==





\section{Introduction}

Large Language Models (LLMs)~\cite{agarwal2025gpt,yang2025qwen3,liu2025deepseek} have been one of the pioneering forces in shaping the deep learning landscape for the past decade.
Pretrained on vast corpus from the Internet, LLMs exhibit strong performance on various downstream applications, such as math~\cite{}, coding~\cite{}, common sense reasoning~\cite{}, and complex tasks that requires systematic reasoning~\cite{}.
Some works also investigate their capacity of handling vision~\cite{}, audio~\cite{}, recommendation~\cite{}, and other modalities' data.
In recent years, agents~\cite{} also emerge as a promising direction of LLMs. 
Based on the capability of foundation LLMs, they can help individuals solve complex real-world tasks such as writing code snippets, analyzing stocks, and even build delicate apps.




Despite their magnificent power, LLMs are still subjected by their Achilles' heel: the computational cost of the vanilla softmax attention~\cite{vaswani2017attention}.
While granting LLMs with detailed historical information, vanilla attention brings upon the quadratic cost in auto-regressive decoding.
This greatly hinders LLMs' wider deployment, especially when it comes to exaggerating long sequences scenarios. 
However, excessive memory in multi-round conversations and accurate retrieval of history contexts are exactly the prerequisite of highly intelligent agents and long chain-of-thought reasoning models.
To further unleash the potential of LLMs and unlock the next level of intelligence, mitigating the bottleneck of attention operation and inventing efficient variants have become destined priority.


Earlier works have explored various efficient solutions of attention.
State space models~\cite{} substitute the growing key and value in attention with a fixed size state as representation of model's historical context, yet fail to match full attention's performance regarding long sequence inputs. 
Sliding variants~\cite{} shift a window~\cite{} or chunk~\cite{} over the sequence and only consider information within that range, but at the risk of overlooking long range history which may also be of vital importance.
Sparse attention~\cite{} selectively choose the most relevant contexts and perform attention operation on that subset of kv cache, which align most closely with our work.
In this work, we aim to resolve the efficiency issue of standard transformers by guiding it to concentrate on most relevant contents while being aware of distant history, which is ensured by a carefully designed summary attention mechanism.

Given the above discussions, we propose \textbf{Kwai Suammry Attention (KSA)}, an efficient, adaptive, and scalable variant of the traditional attention.

==> sections/related_works.tex <==
\section{Related Works}

\subsection{Efficient Attention Variants}
% sliding window

Multi-head attention (MHA)~\cite{vaswani2017attention} has proved itself the cornerstone in deep learning, serving as an indispensable component across language~\cite{2018gpt1,devlin2019bert}, vision~\cite{dosovitskiy2020image,ramesh2021zero}, and video generation~\cite{peebles2023scalable}.

Apart from notable success gained, two factors hinder MHA's further application: 
i) the quadratic cost of computing the full \(N \times N\) attention score matrix during training and long-sequence prefill; and
ii) the linearly growing KV cache that strains memory during auto-regressive generation.
To address these, prior works have explored efficient attention mechanisms along several directions.

The first line of work directly reduces the number of key-value heads to shrink KV cache size.
Multi-query attention (MQA)~\cite{shazeer2019mqa} and grouped-query Attention (GQA)~\cite{ainslie2023gqa} allows multiple query heads to share a single set of key-value heads.
Multi-head Latent Attention (MLA)~\cite{liu2024mla} pushes this further by projecting KV tensors into low-dimensional latent space.
By utilizing matrix absorption technique, only the latent vectors are stored in KV cache during inference, leading to a drastic reduction in memory overhead while retaining expressiveness.

The second category circumvents the quadratic complexity by limiting the attention scope. 
Local attention mechanisms, such as sliding-window and sliding-chunk approaches~\cite{child2019generating,beltagy2020longformer,jiang2023diego,team2024gemma}, restrict each query to attend only to KV states within a window of size \(W\), reducing the complexity from \(\mathcal{O}(N^2)\) to \(\mathcal{O}(W*N)\). 
Sparse attention variants~\cite{yang2026longlive,zhang2025spargeattn,yuan2025native,liu2025dsa} further select a small subset of \(K\) KV tokens based on importance scores and compute attention only over that fraction, yielding \(\mathcal{O}(K*N)\) complexity while preserving long-range details that local attention may miss.



The third direction reformulates attention operation using kernel methods and state-space models.
Kernel-based approximations, such as Retentive Networks~\cite{sun2023retentive} and Eagle~\cite{peng2024eagle}, linearize the softmax function via kernel feature maps or employing hybrid recurrence mechanisms. 
In parallel, state space models like Mamba~\cite{gu2024mamba} and Gated Delta Net~\cite{yang2025gated} model long-range dependencies through a selective, fixed-dimensional hidden state, which offer a different memory mechanism that scales efficiently with context lengths.

However, these solutions still face a performance-efficiency trade-off. 
Sparse attention methods incur memory overhead from KV caches, while linear variants frequently exhibit performance degradation on long-sequence tasks.
To bridge this gap, we propose a novel attention mechanism that elegantly addresses these bottlenecks.
By integrating summary tokens within a hybrid architecture, our approach strikes a favorable balance between modeling expressiveness and inference efficiency.

% Prior works explore various solutions for efficient attention, characterized by local attention~\cite{child2019generating,beltagy2020longformer,jiang2023diego, team2024gemma}, kernel-based approximations~\cite{sun2023retentive,peng2024eagle,gu2024mamba,yang2025gated}, and sparse attention variants~\cite{yang2026longlive,zhang2025spargeattn,yuan2025native,liu2025dsa}.

 
%linear



%mamba SSM



\subsection{Hybrid Attention Architecture}


To better balance the trade-off of efficient and full attention, existing researches mix them in a intra-block hybrid model manner.
Widely accepted practice is to combine one full-attention layer with
several efficient layers, yielding maximized recall with minimum KV-cache cost. 

Small-scale hybrid models include Hybrid-H3~\cite{fu2023hungry} using only two attention layers with up to 2.7B parameters, RecurrentGemma~\cite{botev2024recurrentgemma} using a 2:1 ratio and sliding window attention with 2B and 9B parameters, and Mamba-2-Hybrid  ~\cite{waleffe2024empirical} using a 4:1 ratio with 8B parameters. 

Large-scale demonstrations include Jamba (7:1 Mamba:Transformer)~\cite{lieber2024jamba,team2024jamba} and production models at Character.ai and
MiniMax that converge on a 6–7:1 ratio [11, 25]. 
Variants trade capacity for memory: Zamba shares a single global-attention block across many recurrent blocks [26, 27]; Samba keeps complexity strictly linear by pairing Mamba with sliding-window attention (SWA) [28].
Beyond block-wise mixing, prefill–decode hybrids such as YOCO compress all keys during an O(L) prefill pass and reuse them during decoding, slashing cache by×layer-count [29, 30].
A finer granularity is head-wise mixing: Hymba allocates some attention heads to
softmax and the rest to state-space updates within the same layer, halving cache while preserving accuracy [10].


==> sections/related_works_old.tex <==
\section{Related Works}

\subsection{KV Cache-Efficient Architecture}
% sliding window



%linear



%mamba SSM



\subsection{Hybrid Attention Architecture}

As large language models are increasingly applied to tasks such as long-document understanding, complex reasoning, and code generation, the ability to model long contexts has become an important research focus. Existing work has explored various approaches to extending the effective context length of language models, including improvements to positional encoding, the use of segment-level memory or recurrence, and inference-time strategies for managing long contexts. While these methods alleviate context length limitations to some extent, they generally do not fundamentally address the computational and memory bottlenecks introduced by standard self-attention in long-sequence settings.

In particular, as the context length grows, the storage and memory-access cost of the key--value (KV) cache during autoregressive generation becomes a major factor affecting inference efficiency. Although recent advances in inference systems and hardware-aware optimizations have improved practical performance, attention computation and KV cache management remain core challenges for scaling language models to long contexts.

% \subsection{Efficient Attention}

A large body of work has proposed efficient attention mechanisms to reduce the computational cost of modeling long sequences. These methods typically simplify or approximate the standard attention computation by constraining its range, structure, or representation. Representative approaches include sliding-window or local attention, linear attention, and sparse attention.

Sliding-window and local attention methods restrict each token to attend only to a limited neighborhood, achieving linear complexity with respect to sequence length. However, the limited interaction range constrains representational capacity, as long-range dependencies must be propagated indirectly through multiple layers, which can lead to information degradation over long distances. Linear attention methods reduce complexity by approximating standard attention using kernel functions or feature mappings, but such approximations often limit the expressive power of attention, making it difficult to accurately capture complex long-range relationships. Sparse attention methods reduce computation by selecting subsets of tokens for attention, preserving partial global interactions, but typically require additional routing or selection mechanisms and still maintain the full KV cache during inference, limiting their ability to reduce memory and memory-access costs.

Compared to these approaches, Summary Attention focuses on explicitly compressing historical context within the attention mechanism itself, reducing the effective representation size along the sequence-length dimension. This perspective differs from local, linear, or sparse attention designs and offers an alternative direction for efficient long-sequence modeling.

